Benchmarking fixed-length Fingerprint Representations across different Embedding Sizes and Sensor Types

Traditional minutiae-based fingerprint representations consist of a variable-length set of minutiae. This necessitates a more complex comparison causing the drawback of high computational cost in one-to-many comparison. Recently, deep neural networks have been proposed to extract fixed-length embeddings from fingerprints. In this paper, we explore to what extent fingerprint texture information contained in such embeddings can be reduced in terms of dimension while preserving high biometric performance. This is of particular interest since it would allow to reduce the number of operations incurred at comparisons. We also study the impact in terms of recognition performance of the fingerprint textural information for two sensor types, i.e. optical and capacitive. Furthermore, the impact of rotation and translation of fingerprint images on the extraction of fingerprint embeddings is analysed. Experimental results conducted on a publicly available database reveal an optimal embedding size of 512 feature elements for the texture-based embedding part of fixed-length fingerprint representations. In addition, differences in performance between sensor types can be perceived.

==> tables/emb_dims.tex <==
\begin{adjustbox}{max width=\textwidth}
\begin{threeparttable}
\begin{tabular}{c c c c c c c}
    
    \toprule
    \textbf{Num. dims.} & \textbf{Num. ops.} & \textbf{Reweigthed} & \textbf{FNMR (optical)} & \textbf{FNMR (capacitive)}  \\
    
    \midrule 
    \multirow{2}{*}{32} & \multirow{2}{*}{63} & No &\underline{5.36} \% & \underline{10.60} \% & \\ 
     && Yes & 5.38 \% & 10.73 \% & \\ 
\midrule 
\multirow{2}{*}{32} & \multirow{2}{*}{63} & No &\underline{5.36} \% & \underline{10.60} \% & 1.19 \% & 2.42 \% \\ 
 && Yes & 5.38 \% & 10.73 \% & \underline{1.15} \% & \underline{2.38} \% \\ 
\midrule 
\multirow{2}{*}{64} & \multirow{2}{*}{127} & No &\underline{5.37} \% & \underline{10.49} \% & \underline{1.26} \% & \underline{2.38} \% \\ 
 && Yes & 6.02 \% & 12.08 \% & 1.32 \% & 2.45 \% \\ 
\midrule 
\multirow{2}{*}{128} & \multirow{2}{*}{255} & No &\underline{3.51} \% & \underline{7.91} \% & \underline{1.00} \% & \underline{2.14} \% \\ 
 && Yes & 3.91 \% & 8.40 \% & 1.03 \% & 2.16 \% \\ 
\midrule 
\multirow{2}{*}{256} & \multirow{2}{*}{511} & No &\underline{3.04} \% & \underline{8.19} \% & 0.94 \% & 2.31 \% \\ 
 && Yes & 3.09 \% & 8.48 \% & \underline{0.87} \% & \underline{2.09} \% \\ 
\midrule 
\multirow{2}{*}{512} & \multirow{2}{*}{1023} & No &1.93 \% & 6.02 \% & 0.73 \% & 2.04 \% \\ 
 && Yes & \underline{1.89} \% & \underline{5.39} \% & \underline{0.63} \% & \underline{1.68} \% \\ 
\midrule 
\multirow{2}{*}{1024} & \multirow{2}{*}{2047} & No &2.61 \% & 6.46 \% & 0.97 \% & 2.26 \% \\ 
 && Yes & \underline{2.20} \% & \underline{5.58} \% & \underline{0.74} \% & \underline{1.78} \% \\ 
\midrule 
\multirow{2}{*}{2048} & \multirow{2}{*}{4095} & No &3.91 \% & 9.46 \% & 1.17 \% & 2.51 \% \\ 
 && Yes & \underline{3.80} \% & \underline{8.99} \% & \underline{1.05} \% & \underline{2.22} \% \\ 

    
    \bottomrule
       
\end{tabular} 	
\begin{tablenotes}
  \item Num. dims.: Number of embedding dimensions, Num. ops.: Number of floating point operations per comparison, FNMR: False Non-Match Rate, FMR: False Match Rate
\end{tablenotes}
\end{threeparttable} 
\end{adjustbox}



==> tables/variants.tex <==
\begin{adjustbox}{max width=\textwidth}
\begin{threeparttable}
\begin{tabular}{c c c c c c c}
    
    \toprule
    \textbf{Variant} & \textbf{Num. dims.} & \textbf{Reweigthed} & \textbf{Rank-1 IR. (optical)} & \textbf{FNIR (optical)} & \textbf{Rank-1 IR.  (capacitive)} & \textbf{FNIR (capacitive)}  \\
    
    \midrule 
    \multirow{2}{*}{texture branch} & \multirow{2}{*}{512} & No &94.04 \% & \textbf{\underline{58.83} \%} & 89.99 \% & \textbf{\underline{56.93}} \% \\ 
     & & Yes & \underline{94.87} \% & 59.21 \% & \underline{91.52} \% & 61.97 \% \\ 
    \midrule 
    \multirow{2}{*}{minutia branch} & \multirow{2}{*}{512} & No &93.17 \% & \underline{61.60} \% & 89.88 \% & \underline{60.06} \% \\ 
     & & Yes & \underline{93.36} \% & 64.05 \% & \underline{90.02} \% & 60.53 \% \\ 
    \midrule 
    \multirow{2}{*}{texture and minutia branch} & \multirow{2}{*}{512} & No &\textbf{\underline{95.46} \%} & \underline{59.81} \% & \textbf{\underline{92.20} \%} & \underline{60.55} \% \\ 
     & & Yes & 95.22 \% & 60.37 \% & 91.29 \% & 62.22 \% \\ 
    
    \bottomrule
       
\end{tabular} 	
\begin{tablenotes}
  \item Num. dims.: Number of embedding dimensions, Rank-1 IR.: Rank-1 Identification Rate, FNIR: False Negative Identification Rate, FPIR: False Positive Identification Rate
\end{tablenotes}
\end{threeparttable} 
\end{adjustbox}

==> tables/variants_new.tex <==
\begin{adjustbox}{max width=\textwidth}
\begin{threeparttable}
\begin{tabular}{c c c c }
    
    \toprule
    \textbf{Variant}           & \textbf{N}  & \textbf{R(optical)} & \textbf{R (capacitive)}  \\
    
    \midrule 
    texture branch             & \multirow{3}{*}{512} &94.87 & 91.52  \\ 
    minutiae branch            &                      &93.36 & 90.02 \\ 
    texture and minutia branch &           &95.46 & 92.20 \\ 
    
    \bottomrule
       
\end{tabular} 	
\begin{tablenotes}
  \item R: Rank-1 Identification Rate
\end{tablenotes}
\end{threeparttable} 
\end{adjustbox}
